Evo-RAD: Navigating Rare Retinal Disease Diagnosis via Self-Evolving Agentic Retrieval

Large-scale pretrained foundation models have revolutionized general medical screening, but often falter on rare diseases because such conditions are underrepresented in real-world clinical datasets. While retrieval-augmented diagnosis attempts to mitigate this, conventional static methods frequently succumb to the hubness problem, retrieving visually similar but semantically incorrect common diseases. To address this, we propose Evo-RAD, a self-evolving agentic framework that transforms evidence acquisition into a dynamic decision-making task. We formulate retrieval as a Markov Decision Process (MDP) where a graphbased agent observes the reference set state and executes actions to purge discordant evidence (DELETE), acquire pathologically consistent samples (INSERT), or conclude the evolution (TERMINATE). Optimized via Group Relative Policy Optimization (GRPO) with a homogeneityaware reward, the agent learns to maximize the diagnostic homogeneity of the support reference set. Experiments on retinal disease benchmarks show that Evo-RAD substantially improves rare-disease diagnosis, outperforming retinal foundation models by +21.04%, while also surpassing retrieval-based and parameter-efficient fine-tuning methods by +3.56%. Code is available at https://github.com/SDH-Lab/Evo-RAD.

==> method.tex <==
\section{Method}

\subsection{Overview}
Evo-RAD is a retrieval-augmented diagnosis framework designed for long-tailed retinal disease recognition, where one-shot nearest-neighbor retrieval is vulnerable to the hubness effect and can return visually similar but semantically incorrect evidence. Given a query fundus image \(q\), we first extract its visual embedding \(v_q\) using a frozen retinal foundation model. We then retrieve an initial support set from an external memory \(\mathcal{D}\) via Top-\(K\) similarity search:
\begin{equation}
\mathcal{X}_0 = \{x_1,\ldots,x_K\} \subset \mathcal{D},
\end{equation}
where each reference case \(x\) has a precomputed embedding \(v_x\) and an associated disease label \(y_x\in\mathcal{Y}\).
Instead of directly predicting from \(\mathcal{X}_0\), Evo-RAD treats evidence acquisition as a \emph{self-evolving} process: an agent iteratively edits the active support set \(\mathcal{X}_t\) through three discrete operations---\textsc{DELETE} (remove a discordant/hub reference), \textsc{INSERT} (add a potentially consistent reference from memory), and \textsc{TERMINATE} (stop when evidence becomes sufficiently coherent). This yields an evolved support set \(\mathcal{X}_T\), which is then used to produce the final diagnosis (Sec.~\ref{sec:prediction}).

To make insertion efficient, we additionally maintain a lightweight candidate buffer \(\mathcal{B}\subset\mathcal{D}\) (e.g., a larger pre-retrieved pool) from which insertions are drawn during evolution, avoiding repeated full-database search.

\subsection{Retrieval as a Markov Decision Process}
We formulate the self-evolving retrieval procedure as a Markov Decision Process (MDP)
\(\mathcal{M}=\langle \mathcal{S},\mathcal{A},\mathcal{T},\mathcal{R}\rangle\)~\cite{Sutton1998Reinforcement}.
For each query \(q\), the \emph{environment} maintains the current active support set \(\mathcal{X}_t\subset\mathcal{D}\) and updates it according to the agent's editing action. The \emph{agent} observes a state representation of \(\mathcal{X}_t\) (capturing both query relevance and intra-set consistency) and selects actions to suppress hub-induced distractors while retaining diagnostically consistent references.

\noindent\textbf{\textit{State.}}
At step \(t\), the state \(s_t\in\mathcal{S}\) summarizes the current support set \(\mathcal{X}_t\) with respect to the query \(q\) and the internal coherence of \(\mathcal{X}_t\). We represent \(s_t\) as a graph
\begin{equation}
s_t=(\mathcal{G}_t,\mathbf{H}_t),
\end{equation}
where each node corresponds to a reference case \(x\in\mathcal{X}_t\). The node feature of \(x\) concatenates its frozen visual embedding with a set of retrieval/coherence statistics:
\begin{equation}
h(x)=\big[\, v_x \oplus \phi_{\text{stat}}(x,\mathcal{X}_t,q)\,\big], \qquad
\mathbf{H}_t\in\mathbb{R}^{|\mathcal{X}_t|\times D}.
\end{equation}
In \(\phi_{\text{stat}}\), we include: \textbf{(i)} query affinity \(\operatorname{sim}(v_x,v_q)\); \textbf{(ii)} the retrieval rank of \(x\) (from the initial retrieval or the current set); and \textbf{(iii)} an intra-set semantic density term measuring how well \(x\) agrees with the current consensus of \(\mathcal{X}_t\).

\smallskip
\noindent\textit{Graph topology via expanded clinical semantics.}
To expose fine-grained clinical relations that are not captured by coarse disease labels, we enrich each disease label \(y\in\mathcal{Y}\) with a set of clinical tags \(\text{Tags}(y)\) generated by a large language model (GPT 5.1). For each reference case \(x\), we attach \(\text{Tags}(y_x)\) as text and encode it with the (frozen) VLM text encoder to obtain a semantic embedding \(u_x\). We then define the adjacency matrix \(\mathbf{A}_t\) over the active set by pairwise tag-embedding similarity:
\begin{equation}
(\mathbf{A}_t)_{ij} := \text{sim}(x_i,x_j)
=\frac{u_{x_i}^\top u_{x_j}}{\|u_{x_i}\|_2\,\|u_{x_j}\|_2},
\quad x_i,x_j\in\mathcal{X}_t.
\end{equation}
This construction allows the agent to reason about \emph{intra-set semantic consistency} (which is central to detecting and removing hub-like distractors).

\noindent\textit{\textbf{Action.}}
We define a discrete action space
\begin{equation}
\mathcal{A}=\mathcal{A}_{\text{del}}\cup\mathcal{A}_{\text{ins}} \cup \{a_{\text{term}}\}.
\end{equation}
\textbf{Delete.} For each \(x\in\mathcal{X}_t\), there is an action \(a=\textsc{DELETE}(x)\in\mathcal{A}_{\text{del}}\) that removes \(x\) from \(\mathcal{X}_t\), subject to a minimum-size constraint \(|\mathcal{X}_t|\ge \textit{min\_size}\). \\
\textbf{Insert.} Action \(a=\textsc{INSERT}\in\mathcal{A}_{\text{ins}}\) expands the current set by adding one new reference case from a pre-fetched candidate buffer \(\mathcal{B}\). To keep the action space compact, the environment deterministically chooses the inserted case as the most query-similar candidate not yet in \(\mathcal{X}_t\):
\begin{equation}
x_{\text{ins}}
=\argmax_{x\in\mathcal{B}\setminus \mathcal{X}_t}\operatorname{sim}(v_q,v_x).
\end{equation}
This design lets the agent focus on \emph{when to expand} (learned decision) while using a strong visual prior for \emph{what to insert}. \\
\textbf{Terminate.} Action \(a_{\text{term}}\) stops the evolution once the agent judges \(\mathcal{X}_t\) sufficiently coherent.

\noindent \textbf{\textit{Transition.}}
Given action \(a_t\), the transition \(\mathcal{T}\) updates the support set as
\begin{equation}
\mathcal{X}_{t+1}=
\begin{cases}
\mathcal{X}_t\setminus\{x\}, & a_t=\textsc{DELETE}(x),\\
\mathcal{X}_t\cup\{x_{\text{ins}}\}, & a_t=\textsc{INSERT},\\
\mathcal{X}_t, & a_t=a_{\text{term}}.
\end{cases}
\end{equation}
After updating \(\mathcal{X}_{t+1}\), we reconstruct the state graph \(s_{t+1}=(\mathcal{G}_{t+1},\mathbf{H}_{t+1})\) accordingly.

\noindent\textbf{\textit{Homogeneity-aware Reward.}}
To train the agent to produce diagnostically reliable evidence, we design a homogeneity-aware reward that encourages (1) correct final diagnosis, (2) improved label purity relative to the initial retrieval (counteracting hubness), and (3) higher intra-set semantic density. For a trajectory \(\tau=\{(s_t,a_t)\}_{t=0}^{T}\), we define the total return
\begin{equation}
R(\tau)= R_{\text{traj}}(\mathcal{X}_T) + \sum_{t=0}^{T-1} r_{\text{step}}(s_t,a_t).
\end{equation}

\noindent\textbf{Trajectory-level reward.}
Let \(\hat{y}(\mathcal{X})\) be the diagnosis conditioned on support set \(\mathcal{X}\) (defined in Sec.~\ref{sec:prediction}), and let \(y^\star\) be the ground-truth label of the query during training. We define the label purity
\begin{equation}
\text{Pur}(\mathcal{X})=\frac{1}{|\mathcal{X}|}\sum_{x\in\mathcal{X}}\mathbb{I}[y_x=y^\star],
\end{equation}
and the mean pairwise semantic density based on tag embeddings \(\{u_x\}\):
\begin{equation}
\text{Den}(\mathcal{X})=\frac{2}{|\mathcal{X}|(|\mathcal{X}|-1)}\sum_{i<j}\cos(u_{x_i},u_{x_j}).
\end{equation}
We then define
\begin{equation}
R_{\text{traj}}(\mathcal{X}_T)
=
\alpha\,\mathbb{I}\!\left[\hat{y}(\mathcal{X}_T)=y^\star\right]
+\beta\Big(\text{Pur}(\mathcal{X}_T)-\text{Pur}(\mathcal{X}_0)\Big)
+\gamma\,\text{Den}(\mathcal{X}_T).
\end{equation}

\noindent\textbf{Step-level reward.}
To provide denser feedback while avoiding overly aggressive negative shaping, we adopt a positive-only step reward:
\begin{equation}
r_{\text{step}}(s_t,a_t)=
\eta_{\text{ins}}\;\mathbb{I}\!\left[a_t=\textsc{INSERT}\right]\mathbb{I}\!\left[y_{x_{\text{ins}}}=y^\star\right]
+
\eta_{\text{del}}\;\mathbb{I}\!\left[a_t=\textsc{DELETE}(x_{\text{del}})\right]\mathbb{I}\!\left[y_{x_{\text{del}}}\neq y^\star\right].
\end{equation}
Incorrect insertions/deletions receive zero reward, which stabilizes exploration early in training.

\subsection{Graph Policy Network and GRPO Optimization}
With the MDP defined above, we learn a retrieval-editing policy \(\pi_\theta(a_t \mid s_t)\) that iteratively updates \(\mathcal{X}_t\) toward a coherent evidence set. We parameterize \(\pi_\theta\) with a graph-based policy network and optimize it using Group Relative Policy Optimization (GRPO)~\cite{guo2025deepseek}.

\noindent \textbf{\textit{Graph-based policy network.}}
Given the state graph \(s_t=(\mathcal{G}_t,\mathbf{H}_t)\) with adjacency matrix \(\mathbf{A}_t\), we apply a Graph Convolutional Network (GCN)~\cite{Kipf2016Semi} to propagate semantic-consistency signals among references. With self-loops \(\hat{\mathbf{A}}_t=\mathbf{A}_t+\mathbf{I}\) and degree matrix \(\hat{\mathbf{D}}_t\), the \(l\)-th layer updates node features as
\begin{equation}
\mathbf{H}_t^{(l+1)}=
\sigma\!\left(
\hat{\mathbf{D}}_t^{-\frac{1}{2}}
\hat{\mathbf{A}}_t
\hat{\mathbf{D}}_t^{-\frac{1}{2}}
\mathbf{H}_t^{(l)}\mathbf{W}^{(l)}
\right),
\quad \mathbf{H}_t^{(0)}=\mathbf{H}_t.
\end{equation}
After \(L\) layers (\(L=2\)), we produce action logits by combining node-level deletion scores and graph-level operation scores (insert/terminate):
\begin{equation}
\pi_\theta(a_t\mid s_t)=\operatorname{Softmax}\!\Big(
\Big[
\{\operatorname{MLP}_{\text{local}}(h_x^{(L)})\}_{x\in\mathcal{X}_t},\;
\operatorname{MLP}_{\text{global}}(\operatorname{Pool}(\mathbf{H}_t^{(L)}))
\Big]
\Big)_{a_t},
\end{equation}
where \(\operatorname{Pool}(\cdot)\) is mean pooling and \(\operatorname{MLP}_{\text{local}},\operatorname{MLP}_{\text{global}}\) are two MLP heads.

\noindent \textbf{\textit{GRPO optimization.}}
GRPO eliminates the need for a learned critic by using group statistics as a baseline. For each query \(q\), we sample a group of trajectories \(\mathcal{T}_G=\{\tau_1,\ldots,\tau_G\}\) from \(\pi_{\theta_{\text{old}}}\), compute their returns \(\{R(\tau_i)\}_{i=1}^G\), and form the normalized advantage
\begin{equation}
\hat{A}_i=
\frac{R(\tau_i)-\operatorname{Mean}(\{R(\tau_j)\}_{j=1}^G)}
{\operatorname{Std}(\{R(\tau_j)\}_{j=1}^G)+\epsilon}.
\end{equation}
We then update the policy by maximizing
\begin{equation}
\mathcal{J}(\theta)=
\mathbb{E}_{q}\left[
\frac{1}{G}\sum_{i=1}^G
\left(
\frac{\pi_{\theta}(\tau_i)}{\pi_{\theta_{\text{old}}}(\tau_i)}\hat{A}_i
-\beta\,\mathbb{D}_{\text{KL}}\!\left(\pi_{\theta}(\cdot\mid q)\,\|\,\pi_{\text{ref}}(\cdot\mid q)\right)
\right)
\right],
\end{equation}
where \(\pi_{\text{ref}}\) is a reference policy and the KL term regularizes updates for stability.

\subsection{Evidence-Conditioned Prediction}
\label{sec:prediction}
After the agent terminates, we obtain the evolved support set \(\mathcal{X}_T\). In this work, we use majority voting over the labels of evolved references for diagnosis:
\begin{equation}
\hat{y}
=\argmax_{c\in\mathcal{Y}}
\sum_{x\in\mathcal{X}_T}\mathbb{I}(y_x=c).
\end{equation}
This prediction rule makes the effect of evidence evolution explicit: performance improvements must come from producing a more diagnostically coherent \(\mathcal{X}_T\), rather than modifying the frozen backbone.
